Rethinking Distance Metrics for Counterfactual Explainability

Counterfactual explanations have been a popular method of post-hoc explainability for a variety of settings in Machine Learning. Such methods focus on explaining classifiers by generating new data points that are similar to a given reference, while receiving a more desirable prediction. In this work, we investigate a framing for counterfactual generation methods that considers counterfactuals not as independent draws from a region around the reference, but as jointly sampled with the reference from the underlying data distribution. Through this framing, we derive a distance metric, tailored for counterfactual similarity that can be applied to a broad range of settings. Through both quantitative and qualitative analyses of counterfactual generation methods, we show that this framing allows us to express more nuanced dependencies among the covariates.

==> formatted_figures/Adult_Results/Dataset_table.tex <==
\begin{tabular}{c} 
    Data \\
    \hline
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Adult} \\
    ~ \\
    ~ \\
    ~ \\
    ~\\
\end{tabular}

==> formatted_figures/Adult_Results/Log_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    \multicolumn{6}{c}{Logistic Regression} \\
    \hline
    $l_{0}$ & $l_{2}$ & \texttt{yNN} & \texttt{Redun.} & \texttt{Acc.} & \texttt{t(s)} \\
    \hline
    0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
    A & B & C & D & E & F \\
\end{tabular}

==> formatted_figures/GMSC_Results/Dataset_table.tex <==
\begin{tabular}{c} 
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Heloc} \\
    ~ \\
    ~ \\
    ~ \\
    ~  \\
\end{tabular}

==> formatted_figures/Heloc_Results/Dataset_table.tex <==
\begin{tabular}{c} 
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Heloc} \\
    ~ \\
    ~ \\
    ~ \\
    ~  \\
\end{tabular}

==> formatted_figures/Heloc_Results/Log_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    0.068 & 0.048 & 0.127 & 3.783 & 0.999 & 0.051 \\
    0.067 & 0.048 & 0.126 & 3.871 & 0.999 & 0.069 \\
    0.156 & 0.156 & 0.206 & 19.10 & 1.000 & 0.029 \\
    0.141 & 0.157 & 0.313 & 17.85 & 1.000 & 0.093 \\
    1.197 & 0.074 & 0.7645 & 14.324 & 1.000 & 0.549 \\
    1.378 & 0.812 & 0.991 & 16.436 & 1.000 & 0.858 \\
    0.759 & 0.582 & 0.671 & 11.628 & 0.999 & 0.207 \\
    0.630 & 0.489 & 0.429 & 15.440 & 1.000 & 2.192 \\
\end{tabular}

==> formatted_figures/MagicGT_Results/ANN_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    $l_{2}$ & $l_{\infty}$ & \texttt{yNN} & \texttt{Redun.} & \texttt{t(s)} \\
    \hline
    0.019 & 0.094 & 0.113 & 6.902 & 0.007 \\
    0.028 & 0.067 & 0.125 & 5.818 & 0.003 \\
    0.038 & 0.095 & 0.123 & 4.001 & 0.429 \\
    0.043 & 0.088 & 0.136 & 4.096 & 0.397 \\
    0.488 & 0.480 & 0.545 & 5.920 & 4.289 \\
    0.644 & 0.571 & 0.854 & 8.048 & 3.593 \\
    0.019 & 0.076 & 0.126 & 5.947 & 0.004 \\
    0.023 & 0.085 & 0.151 & 6.752 & 0.022 \\
    0.206 & 0.278 & 1.000 & 9.110 & 0.002 \\
\end{tabular}

==> formatted_figures/MagicGT_Results/Dataset_table.tex <==
\begin{tabular}{c} 
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Heloc} \\
    ~ \\
    ~ \\
    ~ \\
    ~  \\
\end{tabular}

==> formatted_figures/MagicGT_Results/Method_table.tex <==
\begin{tabular}{c} 
    Method \\
    \hline
    Wachter \\
    Wachter (Ours) \\
    Dice \\
    Dice (Ours) \\
    FACE \\
    FACE (Ours)\\
    Growing Spheres \\
    Growing Spheres (Ours) \\
    CCHVAE \\
    CLUE
\end{tabular}

==> formatted_figures/Rice_Results/Ann_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    $l_{2}$ & $l_{\infty}$ & \texttt{yNN} & \texttt{Redun.} & \texttt{Div.} & \texttt{t(s)} \\
    \hline
    \rowcolor[gray]{1.}
    0.091 & 0.118 & 0.18 & 2.466 & - & 0.010 \\
    \rowcolor[gray]{.8}
    0.122 & 0.121 & 0.415 & 2.878 & - & 0.005 \\
    \rowcolor[gray]{1.}
    0.082 & 0.184 & 0.104 & 3.114 & 0.074 & 0.471 \\
    \rowcolor[gray]{.8}
    0.115 & 0.196 & 0.326 & 1.762 & 0.055 & 0.587 \\
    \rowcolor[gray]{1.}
    0.691 & 0.125 & 0.747 & 4.1 & - & 0.405 \\
    \rowcolor[gray]{.8}
    0.258 & 0.255 & 1.000 & 6.3 & - & 0.425 \\
    \rowcolor[gray]{1.}
    0.110 & 0.209 & 0.061 & 2.991 & - & 0.005 \\
    \rowcolor[gray]{.8}
    0.119 & 0.213 & 0.156 & 3.703 & - & 0.039 \\
    \rowcolor[gray]{1.}
    0.192 & 0.241 & 0.502 & 2.332 & - & 0.080 \\
\end{tabular}



==> formatted_figures/Rice_Results/Dataset_Table.tex <==
\begin{tabular}{c} 
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Heloc} \\
    ~ \\
    ~ \\
    ~ \\
    ~  \\
\end{tabular}

==> formatted_figures/Rice_Results/Log_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    0.068 & 0.048 & 0.127 & 3.783 & 0.999 & 0.051 \\
    0.067 & 0.048 & 0.126 & 3.871 & 0.999 & 0.069 \\
    0.156 & 0.156 & 0.206 & 19.10 & 1.000 & 0.029 \\
    0.141 & 0.157 & 0.313 & 17.85 & 1.000 & 0.093 \\
    1.197 & 0.074 & 0.7645 & 14.324 & 1.000 & 0.549 \\
    1.378 & 0.812 & 0.991 & 16.436 & 1.000 & 0.858 \\
    0.759 & 0.582 & 0.671 & 11.628 & 0.999 & 0.207 \\
    0.630 & 0.489 & 0.429 & 15.440 & 1.000 & 2.192 \\
\end{tabular}

==> formatted_figures/WineQuality_Results/ANN_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    $l_{2}$ & $l_{\infty}$ & \texttt{yNN} & \texttt{Redun.} & \texttt{t(s)} \\
    \hline
    0.029 & 0.061 & 0.091 & 3.947 & 0.136 \\
    0.052 & 0.063 & 0.126 & 1.161 & 0.093 \\
    0.033 & 0.072 & 0.143 & 1.239 & 0.479 \\
    0.043 & 0.068 & 0.155 & 1.644 & 0.367 \\
    1.218 & 0.632 & 0.531 & 8.070 & 0.622 \\
    0.957 & 0.543 & 0.632 & 8.631 & 0.622 \\
    0.987 & 0.862 & 0.078 & 8.399 & 0.004 \\
    1.153 & 0.908 & 0.099 & 8.573 & 0.026 \\
    1.253 & 1.000 & 0.2 & 11.967  & 0.004 \\
\end{tabular}


==> formatted_figures/WineQuality_Results/Dataset_table.tex <==
\begin{tabular}{c} 
    ~ \\
    ~ \\
    ~ \\
    ~  \\
    {\footnotesize Heloc} \\
    ~ \\
    ~ \\
    ~ \\
    ~  \\
\end{tabular}

==> formatted_figures/WineQuality_Results/Log_Results.tex <==
\setlength{\tabcolsep}{1em} 
\begin{tabular}{c c c c c c} 
    0.068 & 0.048 & 0.127 & 3.783 & 0.999 & 0.051 \\
    0.067 & 0.048 & 0.126 & 3.871 & 0.999 & 0.069 \\
    0.156 & 0.156 & 0.206 & 19.10 & 1.000 & 0.029 \\
    0.141 & 0.157 & 0.313 & 17.85 & 1.000 & 0.093 \\
    1.197 & 0.074 & 0.7645 & 14.324 & 1.000 & 0.549 \\
    1.378 & 0.812 & 0.991 & 16.436 & 1.000 & 0.858 \\
    0.759 & 0.582 & 0.671 & 11.628 & 0.999 & 0.207 \\
    0.630 & 0.489 & 0.429 & 15.440 & 1.000 & 2.192 \\
\end{tabular}

==> formatted_figures/WineQuality_Results/Method_table.tex <==
\begin{tabular}{c} 
    Method \\
    \hline
    Wachter \\
    Wachter (Ours) \\
    Dice \\
    Dice (Ours) \\
    FACE \\
    FACE (Ours)\\
    CCHVAE
\end{tabular}

==> formatted_figures/fashion_mnist.tex <==
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{ 
        \begin{tabular}{ c c c c c | c c c c c }
                 & \scalebox{1.5}{Reference} & \scalebox{1.5}{$L2$ Distance} & \scalebox{1.5}{Variational Autoencoder} & \scalebox{1.5}{Ours: $\alpha=0.3$} & & \scalebox{1.5}{Reference} & \scalebox{1.5}{$L2$ Distance} & \scalebox{1.5}{Variational Autoencoder} & \scalebox{1.5}{Ours: $\alpha=0.3$}~ \\
                \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{T-shirt $\rightarrow$ Dress}}} &
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_0-3.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_T-shirt-Dress_acc-(1.00).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_T-shirt-Dress_acc-(1.00).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_T-shirt-Dress_acc-(1.00).pdf} &
                ~
                \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{Trouser $ \rightarrow$ Coat}}} &
                ~
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_1-4.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_Trouser-Coat_acc-(0.99).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_Trouser-Coat_acc-(0.99).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_Trouser-Coat_acc-(1.00).pdf} 
                \\
                \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{Pullover $ \rightarrow$ T-shirt}}} &
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_2-0.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_Pullover-T-shirt_acc-(0.98).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_Pullover-T-shirt_acc-(0.98).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_Pullover-T-shirt_acc-(0.98).pdf} &
                ~ 
                \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{Bag $ \rightarrow$ T-shirt}}} &
                ~
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_8-0.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_Bag-T-shirt_acc-(0.96).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_Bag-T-shirt_acc-(0.98).pdf}  &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_Bag-T-shirt_acc-(0.98).pdf}
            \\
               \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{Sandal$ \rightarrow$ Ankle Boot}}} &
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_5-9.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_Sandal-Ankle boot_acc-(0.99).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_Sandal-Ankle boot_acc-(0.99).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_Sandal-Ankle boot_acc-(0.99).pdf} &
    
                \raisebox{14mm}{\rotatebox[origin=c]{0}{ \LARGE{Shirt $\rightarrow$ Pullover}}} &
                 \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ref_6-2.pdf} &
                 ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/wachter_cf_Shirt-Pullover_acc-(0.99).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours2_cf_Shirt-Pullover_acc-(0.98).pdf} &
                ~
                \includegraphics[width=0.3\linewidth]{figures/FashionMnist/ours1_cf_Shirt-Pullover_acc-(0.98).pdf}
    \end{tabular}
    }

    \caption{Example Fashion MNIST counterfactuals with $>0.95$ certainty of the desired class on a trained classifier; Our approach introduces semantically meaningful changes that are closer to prototypical examples for the desired class.}
    \label{fig:fashion_mnist_all}
\end{figure*}
